Convergence of Regret Matching in Potential Games and Constrained Optimization

Regret matching (RM) -- and its modern variants -- is a foundational online algorithm that has been at the heart of many AI breakthrough results in solving benchmark zero-sum games, such as poker. Yet, surprisingly little is known so far in theory about its convergence beyond two-player zero-sum games. For example, whether regret matching converges to Nash equilibria in potential games has been an open problem for two decades. Even beyond games, one could try to use RM variants for general constrained optimization problems. Recent empirical evidence suggests that they -- particularly regret matching$^+$ (RM$^+$) -- attain strong performance on benchmark constrained optimization problems, outperforming traditional gradient descent-type algorithms. We show that RM$^+$ converges to an $\epsilon$-KKT point after $O_\epsilon(1/\epsilon^4)$ iterations, establishing for the first time that it is a sound and fast first-order optimizer. Our argument relates the KKT gap to the accumulated regret, two quantities that are entirely disparate in general but interact in an intriguing way in our setting, so much so that when regrets are bounded, our complexity bound improves all the way to $O_\epsilon(1/\epsilon^2)$. From a technical standpoint, while RM$^+$ does not have the usual one-step improvement property in general, we show that it does in a certain region that the algorithm will quickly reach and remain in thereafter. In sharp contrast, our second main result establishes a lower bound: RM, with or without alternation, can take an exponential number of iterations to reach a crude approximate solution even in two-player potential games. This represents the first worst-case separation between RM and RM$^+$. Our lower bound shows that convergence to coarse correlated equilibria in potential games is exponentially faster than convergence to Nash equilibria.

==> text/testingRMvariants.tex <==
\section{RM Variants}

\begin{enumerate}
    \item gradient descent like algo where we remove direction out of the polytope, and use $1/\eta^2 = \sum_{\tau\le t} \norm{\vu^t}_2^2$
    \item For zero-sum games: PRM+ with $\norm{\vr^t}$ forced to be non-decreasing? (maybe some RVU analysis works.) Along similar line: analyze optimistic GD for zero-sum games with adaptive step sizes as in the previous idea. do we still get things like last-iterate convergence or $1/T$ rate?
    \begin{enumerate}
        \item Simultaneous-update PRM+ without forced nondecreasing regret vector norm does {\em not} converge in iterates \citep{Farina23:Regret} but forcing nondecreasing regrets seems to fix that counterexample (Yes, even with simultaneous updates!)
        \item Optimistic GD converges if both players have {\em small constant step sizes}, but with adaptive step sizes it is possible for one player to have large step size
    \end{enumerate}
    \item if RM works well for nonconvex constrained algo, then we might also use moving averages and second order momentum averages, like AMSgrad does with $m_t$ and $v_t$. Rn, RM only takes the last gradients as a step direction, but maybe you want to instead take a step into a momentum based direction instead that is also informed by past gradients. Maybe not so helpful in zero-sum like \textit{games}
    \item DCFR variant: positive regrets are undiscounted, negative regrets are thresholded at $-\sqrt{\sum_{\tau \le t} \norm{\vu^\tau}_2^2}$? (for stochastic RM). ``We want bad actions to have the chance to get back into play (which is hard to happen with stochastic signals without thresholding), but we also don't want it to happen just because the action was good randomly for a few rounds
    \item from discussion with brian sep 19: the GD variant also works for unconstrained optimization if you do the step size update before the point update (if you include the gradient of the current iteration in the denominator of the current step)
    \item 

\end{enumerate}
